blob loss: instance imbalance aware loss functions for semantic segmentation

Deep convolutional neural networks (CNN) have proven to be remarkably effective in semantic segmentation tasks. Most popular loss functions were introduced targeting improved volumetric scores, such as the Dice coefficient (DSC). By design, DSC can tackle class imbalance, however, it does not recognize instance imbalance within a class. As a result, a large foreground instance can dominate minor instances and still produce a satisfactory DSC. Nevertheless, detecting tiny instances is crucial for many applications, such as disease monitoring. For example, it is imperative to locate and surveil small-scale lesions in the follow-up of multiple sclerosis patients. We propose a novel family of loss functions, \emph{blob loss}, primarily aimed at maximizing instance-level detection metrics, such as F1 score and sensitivity. \emph{Blob loss} is designed for semantic segmentation problems where detecting multiple instances matters. We extensively evaluate a DSC-based \emph{blob loss} in five complex 3D semantic segmentation tasks featuring pronounced instance heterogeneity in terms of texture and morphology. Compared to soft Dice loss, we achieve 5% improvement for MS lesions, 3% improvement for liver tumor, and an average 2% improvement for microscopy segmentation tasks considering F1 score.

==> flow/3_alpha.tex <==
\subsection{TODO  (alpha btx  lightsheet microscopy)}
\noindent\textbf{Dataset \& Segementation Task:} TODO
Alpha-BTX is a marker for neuromuscular junctions in mice. This dataset consists of (TODO number) patches of the size of (TODO size in voxel and um) which were drawn from the leg of a tissue cleared mouse scanned with a lightsheet microscope. The patches were manually annotated using the Arivis 4D VR annotation software (TODO citation??).
\newline

TODO add sources for alpha-btx as a marker

TODO shall we include this?

TODO alpha btx is sparsely labeled therefore volumetry cannot be computed in a meaningful way, furthermore precision is not a good metric as many false positives are actually true positives. The best metric for AlphaBTX is therefore sensitivity.

\noindent\textbf{Procedure:} We train our models following the procedure outlined in \Cref{sec:cnn_training} to compare segmentation performance of our proposed loss functions versus established baselines.
For all trainings of \emph{1000} epochs, we set the initial learning rate to \emph{1e-3} and the batch size to \emph{4}.
The networks are trained on two gpus in parallel using \emph{2} random crops with a patch size of \emph{256x256x32} per batch element.

TODO mention min max normalization


We compare our candidate loss against DICE. [TODO more?]


==> flow/3_cfos.tex <==
\subsection{TODO  (CFOS lightsheet microscopy)}
\noindent\textbf{Dataset \& Segementation Task:} TODO
Rami: ```TODO describe CFOS data (already asked Doris for more info/confirmation)
This dataset consists of (TODO number) of patches taken from a tissue cleared brain stained with cFos, a marker which preserves neuronal activity in tissue cleared mice brains, imaged by a lightsheet microscope with a 4x objective and a resolution of \SI{3}x \SI{3}{\micro\metre}
in x-y direction and \SI{6}{\micro\metre} in z direction at a wavelength of 647 \SI{647}{\nano\metre}.```

\noindent\textbf{Procedure:} We train our models following the procedure outlined in \Cref{sec:cnn_training} to compare segmentation performance of our proposed loss functions versus established baselines.
For all trainings of \emph{500} epochs, we set the initial learning rate to \emph{1e-3} and the batch size to \emph{4}.
The networks are trained on a single GPU using \emph{2} random crops with a patch size of \emph{96x96x64} per batch element.

We compare our candidate loss against DICE. [TODO more?]


TODO mention 0 4000 normalization


==> flow/7_code.tex <==
\subsection{Blob loss implementation}
To maintain anonymity, please find an implementation of \emph{blob loss} on \href{https://pastebin.com/xrCNLdY0}{pastebin}.
Later The code will be released on GitHub (see link in main text).

==> flow/7_discolr.tex <==
\subsection{Learning Rate Ablation on DISCO-MS dataset}

\begin{table}[h!]
\nprounddigits{3}
\npdecimalsign{.}
\centering
\caption{
    Summary of learning rate ablation studies on the DISCO-MS dataset.
    As the initial model trained with soft Dice loss (\emph{dice} fails to provide satisfactory results, we train two further models with reduced learning rate following the heuristics suggested by \cite{bengio2012practical}.
    However, all three models trained with \emph{dice} completely over-segment and, therefore, produce \emph{F1} scores.
    In contrast, the \emph{blob dice} model produces significantly fewer false positives.
}
% \scriptsize
\begin{tblr}{colspec={lcr},colspec={|Q[1.5,c] Q[2.5,c] Q[2.5,c] Q[1,c] | Q[1,c] Q[1,c] Q[1,c] Q[1,c] Q[1,c]|}}
% \begin{tabular}{rrlrrrr}
  \hline
\textbf{dataset} & \textbf{architecture} & \textbf{loss} & \textbf{lr} & \textbf{DSC} & \textbf{SDSC} & \textbf{F1} & \textbf{IS} & \textbf{IP} \\ 
  \hline
MS & \href{https://docs.monai.io/en/stable/networks.html\#basicunet}{\emph{BasicUnet}} & blob dice & 1e-3 & $\numprint{0.5456898724}$  & $\numprint{0.6783278589}$  & $\numprint{0.5894206549}$  & $\numprint{0.7597402597}$      & $\numprint{0.4814814815}$    \\
MS & \href{https://docs.monai.io/en/stable/networks.html\#basicunet}{\emph{BasicUnet}} & dice & 1e-3 & $\numprint{0.09523683643}$ & $\numprint{0.08298497289}$ & $\numprint{0.01239879713}$ & $\numprint{0.8701298701}$      & $\numprint{0.006243884255}$  \\
MS & \href{https://docs.monai.io/en/stable/networks.html\#basicunet}{\emph{BasicUnet}} & dice & 3e-4 & $\numprint{0.01585454894}$ & $\numprint{0.03616793724}$ & $\numprint{0.3791208791}$  & $\numprint{0.8961038961}$      & $\numprint{0.2404181185}$    \\
MS & \href{https://docs.monai.io/en/stable/networks.html\#basicunet}{\emph{BasicUnet}} & dice & 1e-4 & $\numprint{0.00747126907}$ & $\numprint{0.01118405106}$ & $\numprint{0.2278026906}$  & $\numprint{0.8246753247}$      & $\numprint{0.1321540062}$    \\
   \hline
\end{tblr}
\label{tab:disco}
\end{table}

==> flow/short_references_bib <==
% network training
@misc{bengio2012practical,
  title         = {Practical recommendations for gradient-based training of deep architectures},
  author        = {Yoshua Bengio},
  year          = {2012},
  eprint        = {1206.5533},
  archiveprefix = {arXiv},
  primaryclass  = {cs.LG},
}

@inproceedings{berman2018lovasz,
  title     = {The lov{\'a}sz-softmax loss: A tractable surrogate for the optimization of the intersection-over-union measure in neural networks},
  author    = {Berman, Maxim and others},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages     = {4413--4421},
  year      = {2018},
}


@article{bhatia2021proteomics,
  title   = {Proteomics of spatially identified tissues in whole organs},
  journal = {arXiv},
  author  = {Bhatia and others},
  year    = {2021},
}


@misc{bilic2019liver,
  title         = {The Liver Tumor Segmentation Benchmark (LiTS)},
  author        = {Patrick Bilic and others},
  year          = {2019},
  eprint        = {1901.04056},
  archiveprefix = {arXiv},
  primaryclass  = {cs.CV},
}

@article{caicedo2019nucleus,
  title     = {Nucleus segmentation across imaging experiments: the 2018 Data Science Bowl},
  author    = {Caicedo, Juan C and others},
  journal   = {Nature methods},
  volume    = {16},
  number    = {12},
  pages     = {1247--1253},
  year      = {2019},
  publisher = {Nature Publishing Group},
}


% main text
@article{eelbode2020optimization,
  title     = {Optimization for medical image segmentation: theory and practice when evaluating with Dice score or Jaccard index},
  author    = {Eelbode, Tom and others},
  journal   = {IEEE Transactions on Medical Imaging},
  volume    = {39},
  number    = {11},
  pages     = {3679--3690},
  year      = {2020},
  publisher = {IEEE},
}

@article{elliott2019slowly,
  title     = {Slowly expanding/evolving lesions as a magnetic resonance imaging marker of chronic active multiple sclerosis lesions},
  author    = {Elliott, Colm and others},
  journal   = {Multiple Sclerosis Journal},
  volume    = {25},
  number    = {14},
  pages     = {1915--1925},
  year      = {2019},
  publisher = {SAGE Publications Sage UK: London, England},
}

@article{falk2019u,
  title     = {U-Net: deep learning for cell counting, detection, and morphometry},
  author    = {Falk, Thorsten and others},
  journal   = {Nature methods},
  volume    = {16},
  number    = {1},
  pages     = {67--70},
  year      = {2019},
  publisher = {Nature Publishing Group},
}


@inproceedings{fidon2017generalised,
  title        = {Generalised wasserstein dice score for imbalanced multi-class segmentation using holistic convolutional networks},
  author       = {Fidon, Lucas and others},
  booktitle    = {International MICCAI Brainlesion Workshop},
  pages        = {64--76},
  year         = {2017},
  organization = {Springer},
}

@article{geirhos2018imagenet,
  title   = {ImageNet-trained CNNs are biased towards texture; increasing shape bias improves accuracy and robustness},
  author  = {Geirhos, Robert and others},
  journal = {arXiv preprint arXiv:1811.12231},
  year    = {2018},
}

@article{goodfellow2014explaining,
  title   = {Explaining and harnessing adversarial examples},
  author  = {Goodfellow, Ian J and Shlens, Jonathon and Szegedy, Christian},
  journal = {arXiv preprint arXiv:1412.6572},
  year    = {2014},
}

% https://arxiv.org/pdf/1206.5533.pdf

@inproceedings{hatamizadeh2022unetr,
  title     = {Unetr: Transformers for 3d medical image segmentation},
  author    = {Hatamizadeh, Ali and others},
  booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages     = {574--584},
  year      = {2022},
}

@inproceedings{he2017mask,
  title     = {Mask r-cnn},
  author    = {He, Kaiming and others},
  booktitle = {Proceedings of the IEEE international conference on computer vision},
  pages     = {2961--2969},
  year      = {2017},
}

@article{isensee2019nnu,
  title     = {nnu-net: Breaking the spell on successful medical image segmentation},
  author    = {Isensee, Fabian and others},
  journal   = {arXiv preprint arXiv:1904.08128},
  volume    = {1},
  pages     = {1--8},
  year      = {2019},
  publisher = {Apr},
}

@article{isensee2021nnu,
  title     = {nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation},
  author    = {Isensee, Fabian and Jaeger, Paul F and Kohl, Simon AA and Petersen, Jens and Maier-Hein, Klaus H},
  journal   = {Nature methods},
  volume    = {18},
  number    = {2},
  pages     = {203--211},
  year      = {2021},
  publisher = {Nature Publishing Group},
}

@article{jungo2021pymia,
  title     = {pymia: A Python package for data handling and evaluation in deep learning-based medical image analysis},
  author    = {Jungo, Alain and et al},
  journal   = {Computer methods and programs in biomedicine},
  volume    = {198},
  pages     = {105796},
  year      = {2021},
  publisher = {Elsevier},
}

@misc{kofler2021using,
  title         = {Are we using appropriate segmentation metrics? Identifying correlates of human expert perception for CNN training beyond rolling the DICE coefficient},
  author        = {Florian Kofler and others},
  year          = {2021},
  eprint        = {2103.06205},
  archiveprefix = {arXiv},
  primaryclass  = {eess.IV},
}

@article{kofler2022approaching,
  title   = {Approaching Peak Ground Truth},
  author  = {Kofler, Florian and Wahle, Johannes and Ezhov, Ivan and Wagner, Sophia and Al-Maskari, Rami and Gryska, Emilia and Todorov, Mihail and Bukas, Christina and Meissen, Felix and Peng, Tingying and others},
  journal = {arXiv preprint arXiv:2301.00243},
  year    = {2022},
}

@misc{kurakin2016adversarial,
  title  = {Adversarial examples in the physical world},
  author = {Kurakin, Alexey and Goodfellow, Ian and Bengio, Samy and others},
  year   = {2016},
}

@inproceedings{lin2017focal,
  title     = {Focal loss for dense object detection},
  author    = {Lin, Tsung-Yi and others},
  booktitle = {Proceedings of the IEEE international conference on computer vision},
  pages     = {2980--2988},
  year      = {2017},
}


@article{ma2021loss,
  title     = {Loss odyssey in medical image segmentation},
  author    = {Ma, Jun and others},
  journal   = {Medical Image Analysis},
  pages     = {102035},
  year      = {2021},
  publisher = {Elsevier},
}

@inproceedings{milletari2016v,
  title        = {V-net: Fully convolutional neural networks for volumetric medical image segmentation},
  author       = {Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle    = {2016 fourth international conference on 3D vision (3DV)},
  pages        = {565--571},
  year         = {2016},
  organization = {IEEE},
}

@article{misra2019mish,
  title   = {Mish: A self regularized non-monotonic neural activation function},
  author  = {Misra, Diganta},
  journal = {arXiv preprint arXiv:1908.08681},
  year    = {2019},
}

@article{pan2019deep,
  title     = {Deep learning reveals cancer metastasis and therapeutic antibody targeting in the entire body},
  author    = {Pan, Chenchen and others},
  journal   = {Cell},
  volume    = {179},
  number    = {7},
  pages     = {1661--1676},
  year      = {2019},
  publisher = {Elsevier},
}

@inproceedings{rahman2016optimizing,
  title        = {Optimizing intersection-over-union in deep neural networks for image segmentation},
  author       = {Rahman, Md Atiqur and Wang, Yang},
  booktitle    = {International symposium on visual computing},
  pages        = {234--244},
  year         = {2016},
  organization = {Springer},
}

@inproceedings{ronneberger2015u,
  title        = {U-net: Convolutional networks for biomedical image segmentation},
  author       = {Ronneberger, Olaf and others},
  booktitle    = {International Conference on Medical image computing and computer-assisted intervention},
  pages        = {234--241},
  year         = {2015},
  organization = {Springer},
}

@inproceedings{salehi2017tversky,
  title        = {Tversky loss function for image segmentation using 3D fully convolutional deep networks},
  author       = {Salehi, Seyed Sadegh Mohseni and Erdogmus, Deniz and Gholipour, Ali},
  booktitle    = {International workshop on machine learning in medical imaging},
  pages        = {379--387},
  year         = {2017},
  organization = {Springer},
}

@inproceedings{shirokikh2020universal,
  title        = {Universal loss reweighting to balance lesion size inequality in 3d medical image segmentation},
  author       = {Shirokikh, Boris and others},
  pages        = {523--532},
  year         = {2020},
  organization = {Springer},
}

@inproceedings{shit2021cldice,
  title     = {clDice-a Novel Topology-Preserving Loss Function for Tubular Structure Segmentation},
  author    = {Shit, Suprosanna and others},
  booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages     = {16560--16569},
  year      = {2021},
}

@article{sirinukunwattana2015stochastic,
  title     = {A stochastic polygons model for glandular structures in colon histology images},
  author    = {Sirinukunwattana, Korsuk and Snead, David RJ and Rajpoot, Nasir M},
  journal   = {IEEE transactions on medical imaging},
  volume    = {34},
  number    = {11},
  pages     = {2366--2378},
  year      = {2015},
  publisher = {IEEE},
}

@incollection{sudre2017generalised,
  title     = {Generalised dice overlap as a deep learning loss function for highly unbalanced segmentations},
  author    = {Sudre, Carole H and others},
  booktitle = {Deep learning in medical image analysis and multimodal learning for clinical decision support},
  pages     = {240--248},
  year      = {2017},
  publisher = {Springer},
}

@article{william_silversmith_2021_5535251,
  author    = {William Silversmith},
  title     = {{seung-lab/connected-components-3d: Zenodo Release v1}},
  journal   = {Zenodo},
  month     = sep,
  year      = 2021,
  publisher = {Zenodo},
  version   = {3.2.1},
  doi       = {10.5281/zenodo.5535251},
  url       = {https://doi.org/10.5281/zenodo.5535251},
}

@article{wright2021ranger21,
  title   = {Ranger21: a synergistic deep learning optimizer},
  author  = {Wright, Less and Demeure, Nestor},
  year    = {2021},
  journal = {arXiv preprint arXiv:2106.13731},
}


@article{zhang2021all,
  title     = {ALL-Net: Anatomical information lesion-wise loss function integrated into neural network for multiple sclerosis lesion segmentation},
  author    = {Zhang, Hang and others},
  journal   = {NeuroImage: Clinical},
  pages     = {102854},
  year      = {2021},
  publisher = {Elsevier},
}

@article{zhao2020cellular,
  title     = {Cellular and molecular probing of intact human organs},
  author    = {Zhao, Shan and others},
  journal   = {Cell},
  volume    = {180},
  number    = {4},
  pages     = {796--812},
  year      = {2020},
  publisher = {Elsevier},
}


@article{zhu2019anatomynet,
  title     = {AnatomyNet: deep learning for fast and fully automated whole-volume segmentation of head and neck anatomy},
  author    = {Zhu, Wentao and others},
  journal   = {Medical physics},
  volume    = {46},
  number    = {2},
  pages     = {576--589},
  year      = {2019},
  publisher = {Wiley Online Library},
}

